Safe Exploration by Solving Early Terminated MDP

Safe exploration is crucial for the real-world application of reinforcement learning (RL). Previous works consider the safe exploration problem as Constrained Markov Decision Process (CMDP), where the policies are being optimized under constraints. However, when encountering any potential dangers, human tends to stop immediately and rarely learns to behave safely in danger. Motivated by human learning, we introduce a new approach to address safe RL problems under the framework of Early Terminated MDP (ET-MDP). We first define the ET-MDP as an unconstrained MDP with the same optimal value function as its corresponding CMDP. An off-policy algorithm based on context models is then proposed to solve the ET-MDP, which thereby solves the corresponding CMDP with better asymptotic performance and improved learning efficiency. Experiments on various CMDP tasks show a substantial improvement over previous methods that directly solve CMDP.

==> fig/ICML20-RL/0_abstract.tex <==
% !TEX root = ICML20_ESPD.tex
\begin{abstract}
Solving the Goal-Conditioned Reward Sparse (GCRS) task is a challenging reinforcement learning problem due to the sparsity of reward signals. This work proposes a new formulation of GCRS tasks under the perspective of the drifted random walk in the state space. Based on the formulation we design a novel method called Evolutionary Stochastic Policy Distillation (ESPD) to solve GCRS tasks by reducing the First Hitting Time of the stochastic process. As a self-imitate approach, ESPD learns a target policy efficiently from a series of its stochastic-variant behaviors in a supervised learning manner. ESPD follows an evolutionary paradigm that applies perturbations upon the action of the target policy as the behavior policy for generating diverse experiences and then selects the superior experiences. Finally the target policy is updated by policy distillation on the selected experience transitions. The experiments on the OpenAI Fetch benchmarks show the improved sample efficiency of the proposed method.\footnote{Code is attached in the supp and will be made publicly available.}
% As an off-policy approach, our method can be further accelerated with distributed training, realizing the capability for future large-scale applications.
 
% \footnote[2]{Code will be made publicly available soon.}
%
%Solving goal-oriented reward sparse (GORS) problem is an important but challenging task in reinforcement learning, In those tasks, the goal is provided to be combined with the current state as the input of a policy.  And a non-trivial positive reward will only be assigned when the agent reach the goal. 
%In this work, we propose a new self-imitate approach as an alternative for normal reinforcement learning approaches. 
%We provide a new formulation of GORS problems from the perspective of drifted random walk on the state space, and propose a practical method, the Evolutionary Stochastic Policy Distillation (ESPD), as a novel approach of such problems. 
%ESPD enables a target policy learns from a series of its stochastic variants through the technique of policy distillation, which can be interpreted as evolution strategy that apply perturbations directly on the action space instead of on the parameter space. 
%And the evolution of our agent can also be regarded as learning with implicit curriculum. Our empirical results based on the MuJoCo GORS control suite shows the high learning efficiency of the proposed method. 
%As an off-policy approach, our method can be accelerate with MPI to further reduce the wall-clock time, providing the capability of future large-scale application.
\end{abstract}


==> fig/ICML20-RL/1_introduction.tex <==
% !TEX root = ICML20_ESPD.tex
\section{Introduction} 
% Although Reinforcement Learning (RL) has been applied to various challenging tasks and outperforms human in most cases~\cite{mnih2015human,silver2016mastering,lillicrap2015continuous,vinyals2019grandmaster,pachockiopenai}, manual effort is still needed to provide sufficient learning signals beside the original \textit{Win or Loss} reward signal~\cite{vinyals2019grandmaster}. In most real-world RL tasks, the rewards are usually extremely sparse.
% % \bz{i think the following logic to the previous sentence is wrong, you already updated the first sentence so the second sentence needs update too!}
% While hindering the learning process, the reward sparsity also provides the flexibility of learning different policies as different solutions to a certain task in order to get rid of deceptive sub-optimal solutions produced by manually designed rewards~\cite{plappert2018multi}. 

Goal-Conditioned Reward Sparse (GCRS) task is one of the challenging reinforcement learning tasks with extremely sparse rewards. In the task, the goal is combined with the current state as the policy input, while the agent is able to receive a positive reward only when the goal is achieved. In many cases, the GCRS task is also considered as the Multi-Goal task where the goal is not fixed and can be anywhere in the state space. 
Therefore the policy has to learn a general solution that can be applied to a set of similar tasks. 
For example, robotic object grasping is such a GCRS task: the target object could be anywhere on the table, the robot has to adjust its arm to reach the object and then grasp it. 
The objective of learning such a policy is to find a feasible path from the current state to the goal~\cite{tamar2016value}. Similar tasks include the Multi-Goal benchmarks in robotics control~\cite{plappert2018multi}.


In previous works, reward shaping \cite{ng1999policy}, hierarchical reinforcement
learning~\cite{dietterich2000hierarchical,barto2003recent}, curriculum
learning~\cite{bengio2009curriculum}, and learning from demonstrations~\cite{schaal1997learning,atkeson1997robot,argall2009survey,hester2018deep,nair2018overcoming}
were proposed to tackle the challenges of learning through sparse rewards. These approaches provide manual guidance from different perspectives. Besides, the Hindsight Experience Replay (HER)~\cite{kaelbling1993learning,NIPS2017_7090} was proposed
to relabel failed trajectories and assign hindsight credits as complementary to the primal sparse
rewards, which is still a kind of Temporal Difference learning and relies on the value of reward.
Recently the Policy Continuation with Hindsight Inverse Dynamics (PCHID)~\cite{sun2019policy} is proposed
to learn with hindsight experiences in a supervised learning manner, but the sample efficiency is still limited by the explicit curriculum setting.


In this work, we aim at improving the sample efficiency and stability of solving these GCRS tasks with an alternative approach based on supervised learning. 
Specifically, by formulating the exploration in GCRS tasks as a random walk in the state space, solving the GCRS task is then equivalent to decreasing the first hitting time (FHT) in the random walk. 
%Based on the Bayesian posterior heuristics: a flipped coin with its front up is with probability $1$ to has its front up at this time, while before the flipping the probability is $0.5$.
The main idea is to encourage the policy producing trajectories that have shorter FHTs. With such a self-imitation manner, the policy learns to reach more and more \emph{hindsight goals}~\cite{NIPS2017_7090} and becomes more knowledgeable to extrapolate its skills to solve the task.
% And as successful trajectories which have short FHT are more likely from a good policy, learning to reproduce such trajectories can improve the target policy if the target policy itself perform poorly at present.
% we can apply self-imitate learning to reproduce the success of reaching a \emph{hindsight goal}~\cite{NIPS2017_7090}, \ie, distilling knowledge from the subset of random samples that conform to certain hindsight target. 
Based on this formulation, we propose a new method for the GCRS tasks, which conforms a self-imitation
learning approach and is independent of the rewards. Our agent learns from its own success or
hindsight success, and extrapolates its knowledge to new situations, enabling the learning
process to be executed in a much more efficient supervised learning manner. 
%Our proposed method, Evolutionary Stochastic Policy Distillation (ESPD), 

\begin{figure*}[t]
\centering
\begin{minipage}[htbp]{0.80\linewidth}
			\centering
			\includegraphics[width=0.9\linewidth]{figures/fig1.pdf}
		\end{minipage}%
\caption{Illustration of Evolutionary Stochastic Policy Distillation. The behavior policy $\pi_B$ is composed of a deterministic policy $\pi_T$ and a stochastic term $\tilde{\eta}$ for exploration. We first generate a batch of trajectories with $\pi_B$, and then use a SELECT function to select the transitions finished by $\pi_B$ in shorter FHT than $\pi_T$ and store the corresponding HIDs in a buffer. Finally, we improve $\pi_T$ with supervised learning and then use the updated policy to generate new samples.}
\label{fig0}
\end{figure*}


We summarize our contributions as follows:
\begin{enumerate}
    \item By modeling the GCRS tasks as random walks in the state space, we provide a novel Stochastic Differential Equation (SDE) formulation of policy learning and bridge the connection between policy improvement and the reduction of FHT.
    \item To reduce the FHT from the SDE perspective, we propose a new method called Evolutionary Stochastic Policy Distillation (ESPD), which combines the mechanism of Evolution Strategy and Policy Distillation, as a self-imitation learning approach for the GCRS tasks.
    \item We demonstrate the proposed method on the Fetch robotics benchmark and show our method can work in isolation to solve GCRS tasks with an improved sample efficiency than previous methods HER and PCHID.
\end{enumerate}

==> fig/ICML20-RL/2_preliminaries.tex <==
% !TEX root = ICML20_ESPD.tex

\section{Preliminaries}

\noindent \textbf{Markov Decision Process.}
We consider a Markov Decision Process (MDP) denoted by a tuple $\mathcal{M}$ containing $(\mathcal{S}, \mathcal{A}, \mathcal{R},\mathcal{T},\gamma, d_{s_0})$, where $\mathcal{S}$ is a finite continuous state space, $\mathcal{A}$ denotes the finite continuous action space, $\mathcal{R}$ is the reward function, where in this work we focus on a special case where the reward function is binary, i.e., tasks with sparse reward. The transition distribution is in general given by $\mathcal{P}(s_{t + 1}| s_t, a_t)$, but in this work, we consider the deterministic dynamics which can be simplified as a mapping of $\mathcal{T}:\mathcal{S}\times\mathcal{A}\to\mathcal{S}$. Discount factor is denoted by $\gamma \in [0, 1]$ and $d(s_0)$ is the start state distribution.
Given a policy $\pi(a|s)$, let
$J(\pi) = \mathbb{E}_{\pi}[\sum_{t=0}^T \gamma^t r(s_t)]$ denote the discounted expected
return, and an optimal policy $\pi^* = \arg \max_\pi J(\pi)$ maximizes that return.


\noindent \textbf{Universal Value Function Approximator and Multi-Goal RL.}
%\subsection{Universal Value Function Approximators}
The Universal Value Function Approximator (UVFA)~\cite{pmlr-v37-schaul15} extends the state space
of \textit{Deep Q-Networks (DQN)}~\cite{mnih2015human} to include goal state as part of
the input, which is useful in the setting where there are multiple goals to achieve. 
Moreover, In the work of Schaul et al.~\cite{pmlr-v37-schaul15} it is shown that in the UVFA setting, the learned policy
can be generalized to previous unseen state-goal pairs. Specifically, let $\mathcal{S}_{(S,G)} = \mathcal{S} \times \mathcal{G}$
denote the \textit{extended state space} of $\mathcal{M}$ where $\mathcal{G}$ is a finite goal space. Normally, a representation mapping $m(\cdot): \mathcal{S}\to\mathcal{G}$ is assumed to be known in such 
multi-goal RL frameworks~\citep{plappert2018multi}.
%The goal is fixed within an episode, namely the induced transition $T'$ satisfies
%$T'((s, g), a) = (T(s, a), g).$
Since the goal is fixed within an episode, the transition function $\mathcal{T}': \mathcal{S}_{(S,G)} \times \mathcal{A} \to \mathcal{S}_{(S,G)}$ 
on the extended state space can be induced from the original transition $\mathcal{T}$ as
$\mathcal{T}'((s, g), a) = (\mathcal{T}(s, a), g).$
 Hence, in order to achieve the goal $g$, the agent
must reach a certain state $s_g$ such that $g = m(s_g)$.


\noindent \textbf{Hindsight Experience Replay.}
Learning with sparse rewards in RL problems remains challenging due to that it is difficult to reach the reward through random explorations. Hindsight Experience Replay (HER) proposes to relabel the failed rollouts as successful ones~\cite{NIPS2017_7090} as a method to deal with the goal-oriented sparse reward problem. The agent in HER receives a reward when reaching either the original goal or the relabeled goal in each episode by storing both original transition pairs $((s_t,g),a_t,(s_{t+1},g),r)$ and relabeled transitions $((s_t,g'),a_t,(s_{t+1},g'),r')$ in the replay buffer, where $g'$ is a certain hindsight goal that will be visited in the following steps, i.e., there exist $k$ such that $g' = m(s_{t+k})$, and $r'$ is the hindsight reward, which will be $+1$ when the hindsight goal is achieved.

%\subsection{Self-Supervised Method with Hindsight}
% \subsection{Policy Continuation with Hindsight Inverse Dynamics}
% As a method revises the collected transition tuple, HER still follows the normal learning paradigm of policy gradient methods. However, as the data collected is extremely off-policy, they are generated through manual relabeling rather than collected by the behavior policy, the learning may suffers from extrapolation error~\citep{fujimoto2019off}. A recent method of Policy Continuation with Hindsight Inverse Dynamics (PCHID)~\citep{sun2019policy} provides a self-supervised approach of using the hindsight knowledge.

% Specifically, PCHID is composed by two components: namely the one-step Hindsight Inverse Dynamics (HID) which enables the self-supervised policy updates, and Policy Continuation (PC) that extends HID to multi-step settings. Their TEST function provides a link between PC and HID.


% \begin{definition}{\bfseries Hindsight Inverse Dynamics.}
% The one-step HID is defined over a series of collected transition trajectories $\{(s_0,g),a_0,r_0,(s_1,g),a_1,...,(s_T,g),a_T,r_T\}_i, i=1,2,...$, by substituting the original goal $g$ with hindsight ones $g' = m(s_{t+1})$ and result in  $\{(s_0,m(s_1)),a_0,(s_1,m(s_2)),a_1,...,(s_{T-1},m(s_{T})),a_{T-1}\}_i$, $i\in\{1,2,...,n\}$. Then HID learns to predict $a_t$ for each given $(s_{t},m(s_{t+1}))$ pair with supervised learning, e.g., optimize the parameters $\theta_{\pi}$ of policy network by:
% \footnotesize
% 	\begin{equation}
% 	\label{eq11}
% 	\theta_{\pi} = \arg\min_\theta
% 	\sum_{s_t,s_{t+1},a_t}||f_\theta((s_t,m(s_{t+1})),(s_{t+1},m(s_{t+1})))-a_t||^2
% 	\end{equation}
% \end{definition}

% While the one-step HID is guaranteed to be optimal, the generalization ability is limited. PCHID then proposes to test the optimality of multi-step HID through a TEST function. Assuming the $1$-step HID policy is optimized and is able to solve all $1$-step solvable tasks, the following $2$-step HID data can be collected using the learned $1$-step HID as an optimal policy. Here the definition of $k$-step solvability defined as
% \begin{definition}{\bfseries $k$-Step Solvability.}
% Given a task ${(s, g)}$, i.e., a state-goal pair, of a certain system with deterministic dynamics,
% we call $(s, g)$ is $k$-step solvable with the optimal policy $\pi$ if the goal $g$ can be achieved
% from $(s, g)$ in exactly $k$ steps under $\pi$, \ie, set $s_{g,0} = (s, g)$ and
% $s_{g,{t + 1}} = \mathcal{T}'(s_{g,t}, \pi(s_{g,t})) = (s_{t + 1}, g)$ for $t \geq 0$, such that $m(s_{k}) = g$.
% %We call a task $\mathcal{M'}$ is $k$-step solvable with $\pi$ if any
% %$\mathcal{M}_{(s, g)} \subset \mathcal{M}'$ is $k$-step solvable with $\pi$. Specifically, if $\pi$ is the
% %optimal policy of $\mathcal{M'}$, we simply call $\mathcal{M'}$ is $k$-step solvable.
% \end{definition}

% So on and so forth, the $k$-step HID transition pairs can be collected gradually, i.e., the learning is explicitly conducted as the $k+1$-step optimality can only be tested once the learning of $k$-step HID converges.
% PCHID then introduces the concept of PC to gradually learn those multi-step HID, by learning those progressively collected HID data in a joint-training manner.

% \begin{definition}{\bfseries Policy Continuation.}
% 	Suppose $\pi$ is a policy function defined on a non-empty sub-state-goal-space $\mathcal{S}_{U}$ of the state space $\mathcal{S}_{(S,G)}$, i.e., $\mathcal{S}_{U}\subset\mathcal{S}_{(S,G)}$. If $\mathcal{S}_{V}$ is a larger subset of $\mathcal{S}_{(S,G)}$, containing $\mathcal{S}_{U}$, i.e., $\mathcal{S}_{U}\subset\mathcal{S}_{V}$ and $\Pi$ is a policy function defined on $\mathcal{S}_{V}$ such that
% 	$\Pi(s) = \pi(s) \forall s\in\mathcal{S}_U $
% 	then we call $\Pi$ a policy continuation of $\pi$, or we can say the restriction of $\Pi$ to $\mathcal{S}_{U}$ is the policy function $\pi$.
% \end{definition}

%  PCHID enables the agent to perform supervised learning from experience replay as long as the trajectory is optimal.
 
% \begin{theorem}
% If $\pi$ is an optimal policy of sub-task $\mathcal{M}_\mathcal{Q'}$,
% then there exists an optimal policy $\Pi$ of $\mathcal{M}_\mathcal{Q''} \supset \mathcal{M}_\mathcal{Q'}$
% such that $\Pi$ is a policy continuation of $\pi$.
% \end{theorem}
% \begin{proof}
% Let $\Pi'$ be an optimal policy of $\mathcal{M}_\mathcal{Q''}$ and construct $\Pi$ as follows:
% \begin{align}
% \Pi(q) = \begin{cases}
% \pi(q) & \mathrm{if\ } q \in \mathcal{Q}'_\pi\\
% \Pi'(q) & \mathrm{otherwise.}
% \end{cases}
% \end{align}
% It is straightforward to see that $\Pi$ is the optimal policy continuation of $\pi$.
% \end{proof}
%The above theorem is simple yet powerful. 

%PCHID enables the agent to perform supervised learning from experience replay as long as the trajectory is optimal.

% \begin{definition}{\bfseries Policy Continuation}
% Given a policy $\pi$ defined on the sub-task $\mathcal{M}_\mathcal{Q'}$ and a policy $\Pi$ defined on the
% sub-task $\mathcal{M}_\mathcal{Q''} \supset \mathcal{M}_\mathcal{Q'}$, we call $\Pi$ is a policy continuation
% of $\pi$, if $\Pi(q) = \pi(q),\ \forall q \in \mathcal{Q}'_\pi$,
% where $\mathcal{Q}'_\pi$ is the set of all extended states reachable by $\pi$ within task $\mathcal{M}_{\mathcal{Q}'}$

% \end{definition}


% \subsection{Policy Continuation}
% %\subsection{Multi-Goal RL and PCHID}
% Most multi-goal RL tasks have sparse rewards. In order to motivate the agent to reach the goal efficiently,
% the reward function $r(s, g)$ is usually set non-negative if $g = m(s)$ while there is a \emph{negative} penalty  
% otherwise. Such a reward distribution can exhibit optimal substructure of the policy.
% \begin{definition}{\bfseries Policy Continuation}
% Given a policy $\pi$ defined on the sub-task $\mathcal{M}_\mathcal{Q'}$ and a policy $\Pi$ defined on the
% sub-task $\mathcal{M}_\mathcal{Q''} \supset \mathcal{M}_\mathcal{Q'}$, we call $\Pi$ is a policy continuation
% of $\pi$, if $\Pi(q) = \pi(q),\ \forall q \in \mathcal{Q}'_\pi$,
% where $\mathcal{Q}'_\pi$ is the set of all extended states reachable by $\pi$ within task $\mathcal{M}_{\mathcal{Q}'}$

% \end{definition}
% \begin{theorem}
% If $\pi$ is an optimal policy of sub-task $\mathcal{M}_\mathcal{Q'}$,
% then there exists an optimal policy $\Pi$ of $\mathcal{M}_\mathcal{Q''} \supset \mathcal{M}_\mathcal{Q'}$
% such that $\Pi$ is a policy continuation of $\pi$.
% \end{theorem}
% \begin{proof}
% Let $\Pi'$ be an optimal policy of $\mathcal{M}_\mathcal{Q''}$ and construct $\Pi$ as follows:
% \begin{align}
% \Pi(q) = \begin{cases}
% \pi(q) & \mathrm{if\ } q \in \mathcal{Q}'_\pi\\
% \Pi'(q) & \mathrm{otherwise.}
% \end{cases}
% \end{align}
% It is straightforward to see that $\Pi$ is the optimal policy continuation of $\pi$.
% \end{proof}
% The above theorem is simple yet powerful. It enables the agent to perform supervised learning
% from experience replay as long as the trajectory is optimal for some sub-tasks.
% Nevertheless, in general given a trajectory $\{(s_0, g), a_0, r_0, \cdots, (s_T, g), a_T, r_T\}$
% generated by the policy $\pi$, it is not easy to decide whether $\pi$ is optimal for
% the sub-task $\mathcal{M}_{(s_0, m(s_T))}$. If we further assume the negative reward is a \emph{constant} value,
% \ie the agent should learn to achieve the goal with minimum actions,
% \citet{sun2019policy} proposed to use the partition induced from the $k$-step solvability
% to help decide the sub-task optimality.
% \begin{definition}{\bfseries $k$-Step Solvability}
% Given a sub-task $\mathcal{M}_{(s, g)}$ of a certain system with deterministic dynamics,
% we call $\mathcal{M}_{(s, g)}$ is $k$-step solvable with a policy $\pi$ if the goal $g$ can be achieved
% from $(s, g)$ within $k$ steps under $\pi$, \ie, set $q_0 = (s, g)$ and
% $q_{t + 1} = T'(q_t, \pi(q_t)) = (s_{t + 1}, g)$ for $t \geq 0$, $\exists i \leq k$ such that $m(s_{i}) = g$.
% We call a sub-task $\mathcal{M'}$ is $k$-step solvable with $\pi$ if any
% $\mathcal{M}_{(s, g)} \subset \mathcal{M}'$ is $k$-step solvable with $\pi$. Specifically, if $\pi$ is the
% optimal policy of $\mathcal{M'}$, we simply call $\mathcal{M'}$ is $k$-step solvable.
% \end{definition}
% Consider the partition $\{\mathcal{M}_k\}_{k=1}^K$ of $\mathcal{M}$ where for any $k < K$, $\mathcal{M}_k$
% is the maximal $k$-solvable sub-task. Suppose the agent has learnt the optimal policy $\pi_k$ of $\mathcal{M}_k$,
% it can decide whether a trajectory of length $(k + 1)$ is optimal by testing whether the corresponding
% sub-task is $k$-step solvable. And those trajectories passing the TEST can serve as supervised training samples
% for extending $\pi_k$ to an optimal policy continuation $\pi_{k + 1}$ on $\mathcal{M}_{k + 1}$.


==> fig/ICML20-RL/3_related_work.tex <==
% !TEX root = ICML20_ESPD.tex
\section{Related Work}

\noindent \textbf{Learning with Experts and Policy Distillation.}
% Imitation Learning (IL) approaches introduce expert data in the learning of a
% agent~\cite{pomerleau1991efficient,ross2011reduction}, while similar techniques
% are used in the literature of Learning from Demonstrations
% (LfD)~\cite{atkeson1997robot,schaal1997learning,argall2009survey}, where experience
% of human expert will be collected to help the learning of an agent. Those methods are
% further extended in the setting of Deep Q-learning~\cite{mnih2015human,hester2018deep},
% combined with DDPG~\cite{lillicrap2015continuous,nair2018overcoming} or to learn
% from imperfect expert data~\cite{gao2018reinforcement}.
Policy Distillation (PD) was proposed to extract the policy of a trained RL agent with
a smaller network to improve the efficiency as well as the final performance or
combine several task-specific agents together~\cite{rusu2015policy}. Latter extensions
proposed to improve the learning efficiency~\cite{schmitt2018kickstarting}, enhance
multi-task learning~\cite{teh2017distral,arora2018multi}. All of those methods start from a trained expert agent or human expert experience
that can solve a specific task~\cite{czarnecki2019distilling}. As a comparison, our proposed method focus on extracting knowledge from stochastic behaviors, which is capable to act as a feasible policy itself with regard to the primal task.
In PD, a deterministic teacher policy is provided and can be queried to generate enough data to teach the student policy. However, in ESPD all the teacher policies are unknown as they are \textbf{stochastic variants} of the student policy. We regard those stochastic variants as they are from \textbf{unkonwn deterministic oracle policies} and distill those policies through the single corresponding trajectory. In ESPD, the teacher model is unknown and can not be queried as in PD.


\noindent \textbf{Evolution Strategies and Parameter Noise.}
The Evolution Strategy (ES) was proposed by~\cite{salimans2017evolution} as an alternative
to standard RL approaches, where the prevailing temporal difference based value function
updates or policy gradient methods are replaced as perturbations on the parameter space
to resemble the evolution. Later on, \cite{campos2018importance} improved the efficiency
of ES by means of importance sampling. Besides, the method was also extended to be combined
with Novelty-Seeking to further improve the performance~\cite{conti2018improving}. Thereafter, \cite{plappert2017parameter} proposed to use Parameter Noise as an alternative to the action space noise injection for better exploration. They show such a perturbation
on the parameter space can be not only used for ES methods, but also collected to improve the sample efficiency by combining it with traditional RL methods.
While previous ES algorithms apply perturbations on the parameter noise and keep the
best-performed variates, our approach implicitly execute the policy evolution by distilling
better behaviors, therefore our approach can be regarded as an evolutionary method based on
action space perturbation. 


\noindent \textbf{Supervised and Self-Imitate Approaches in RL.}
Recently, several works put forward to use supervised learning to improve the stability and
efficiency of RL. \cite{zhang2019policy} propose to utilize supervised learning to tackle the
overly large gradients problem in policy gradient methods. In order to improve sample efficiency,
the work chose to first design a target distribution proposal and then used supervised
learning to minimize the distance between present policy and the target policy distribution.
The Upside-Down RL proposed by \cite{schmidhuber2019reinforcement} used supervised
learning to mapping states and rewards into action distributions, and therefore acted as a normal
policy in RL. Their experiments show that the proposed UDRL method outperforms several
baseline methods~\cite{srivastava2019training}. In the work of~\cite{sun2019policy}, a curriculum learning
scheme is utilized to learn policies recursively.
The self-imitation idea relevant to ESPD is also discussed in the concurrent work of~\cite{ghosh2019learning}, but ESPD further uses the SELECT function to improve the quality of collected data for self-imitation learning.

% [Ghosh 2019] Our work differs from this contemporary work mainly in that we apply a TEST function to further improve the quality of relabeled data.
% [Lynch 2019] and [Savinov 2019] are more related to curiosity-driven or intrinsic reward methods.


==> fig/ICML20-RL/4_method.tex <==
% !TEX root = ICML20_ESPD.tex
\section{Method}
\subsection{Problem Formulation}
\begin{figure*}[t]
\centering
\begin{minipage}[htbp]{0.85\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/fig2.pdf}
		\end{minipage}%
\caption{Illustration of the selection process: first we generate episodes with the stochastic behavior policy $\pi_B$, which is composed of the deterministic target policy $\pi_T$ and a noise term drawn from Gaussian, then we check the superiority of generated transitions over the target policy. If $\pi_T$ can not find a shorter path for a transition generated by $\pi_B$, the select function will return True and the transition will be stored for Stochastic Policy Distillation. Therefore, $\pi_T$ will learn to evolve to solve more sub-task, \ie, transitions, continuously.}
\label{illu_fig}
\end{figure*}
In a given goal-oriented reinforcement learning task, we assume there exists an unknown
metric $\mathcal{D}(s_t, g)$ that represents the distance between the current state $s_t$
and the desired goal state $g$. For example $\mathcal{D}(s,g)$ is the Euclidean distance in
barrier-free navigation tasks; or the Manhattan distance in navigation tasks with obstacles.

A feasible solution of the task should be a policy $\pi(s_t,g)$ that outputs an action
$a_t$, such that the distance $\mathcal{D}(s_{t+1},g)\le\mathcal{D}(s_t,g)$ for deterministic
dynamics, or $\mathbb{E}[\mathcal{D}(s_{t+1},g)]\le\mathbb{E}[\mathcal{D}(s_t,g)]$
for stochastic dynamics. 
We assume $\mathcal{D}(s,g)$ is continuous and differentiable on $s$, and
$\mathrm{d}s = -\xi\frac{\partial \mathcal{D}(s,g)}{\partial s} \mathrm{d}t$ is a feasible move, as it decreases the distance between $s$ and $g$ when $\xi$ is sufficiently small. 
We further assume the state is a vector, the state transition $\Delta s_t = s_{t+1} - s_t$ is determined by both the dynamics $\phi_s(\cdot): \mathcal{S}\times\mathcal{A} \rightarrow \Delta \mathcal{S}$ and the action
$a_t = \pi(s_t,g)$ provided by the policy. We may write a sufficient condition for
a feasible policy:
\begin{equation}
    \phi_s(\pi(s,g)) = -\xi\frac{\partial \mathcal{D}(s,g)}{\partial s} \mathrm{d}t,
\end{equation}
we further assume $\phi_s^{-1}(\cdot)$ exists\footnote[2]{The assumption can be released to a existence of pseudo inverse: $\phi_s^{-1}(\phi_s(a)) \in A'$, where $A'$ is a set s.t. $\forall a'\in A'$, $\phi_s(a') = \phi_s(a)$.}, \ie~$\forall a \in \mathcal{A}$,
$\phi_s^{-1}(\phi_s(a)) = a$. Hence, by parameterizing the policy
$\pi(s,g)$ with $\theta$, we have
\begin{equation}
   \pi_\theta(s,g) =  \phi_s^{-1}\left(-\xi\frac{\partial \mathcal{D}(s,g)}{\partial s}\mathrm{d}t\right),
\end{equation}
is a feasible policy, \ie, it tends to solve the GCRS task as it continuously minimizes the distance between the current state and the goal.
The above equation tells us, in order to learn a well-performing policy, the policy should
learn two unknown functions: the inverse dynamics $\phi_s^{-1}(\cdot)$ and the derivatives
of distance metric $\mathcal{D}(\cdot,\cdot)$ over $s$ and $g$ with regard to the state $s$.
The work of~\citet{sun2019policy} proposed PCHID to use Hindsight Inverse Dynamics (HID)
as a practical policy learning method in such GCRS tasks. Specifically, in Inverse Dynamics,
a model parameterized by $\theta$ is optimized by minimizing the mean square error of predicted
action $\hat{a}_t$ and executed action $a_t$ between adjacent states $s_t$ and $s_{t+1}$, \ie
~$\theta = \mathop{\arg\min}_{\theta} (a_t - \hat{a}_t)^2 = \mathop{\arg\min}_{\theta} (a_t - \pi_{\theta}(s_t,s_{t+1}))^2$. The
HID revises the latter $s_{t+1}$ with its goal correspondence $g_{t+1} = m(s_{t+1})$, where the
mapping $m$ is assumed to be known in normal GCRS task settings. $m: {\mathcal{S}}\to \mathcal{G}$
s.t. $\forall s\in{\mathcal{S}}$ the reward function $r(s,m(s)) = 1$. In the single step transition setting, the learning objective of the policy is to learn HID by
\begin{equation}
\label{eq_hid}
    \theta = \mathop{\arg\min}_{\theta} (a_t - \hat{a}_t)^2 = \mathop{\arg\min}_{\theta} (a_t - \pi_{\theta}(s_t,g_{t+1}))^2.
\end{equation}
Eq.\ref{eq_hid} shows the HID can be used to train a policy with supervised learning by minimizing the prediction error. However, to get more capable policy that is able to solve harder cases,
training the policy only with 1-step HID is not enough. The work of PCHID then proposed to check the
optimality of multi-step transitions with a TEST function and learn multi-step HID recursively. Such an explicit curriculum learning strategy is not efficient as multi-step transitions can only be collected after the
convergence of previous sub-policies. 



Here we interpret how PCHID works from the SDE perspective. 
Practically, a policy is always parameterized as a neural network trained from scratch
to solve a given task. At beginning the policy will not be fully goal-oriented as a
feasible policy. With random initialization, the policy network will just perform
random actions regardless of what state and goal are taken as inputs. We use a coefficient
$\epsilon$ to model the goal awareness of the policy, e.g., $\epsilon=0$ denotes a purely random policy, and $\epsilon=1$ denotes a better policy. In order to collect diverse experiences and improve our target policy, we follow traditional RL approaches to assume a random noise term denoted by $N$
with coefficient $\sigma$ to execute exploration. Hence, the behavioral policy becomes:
\begin{equation}
\label{equation_4}
    \pi_{\mathrm{behave}} =\pi_{\theta}(s,g) + \sigma N 
    = \epsilon \phi_s^{-1}\left(-\xi\frac{\partial \mathcal{D}(s,g)}{\partial s}\mathrm{d}t\right) + \sigma N.
\end{equation}
The behavioral policy above combines a deterministic term and a stochastic term, which in
practice can be implemented as a Gaussian noise or OU-noise~\cite{lillicrap2015continuous}. Although we assume a deterministic
policy $\pi_{\theta}(s,g)$ here, the extension to stochastic policies is straightforward, e.g., the network can predict the mean value and the standard deviation of an action to form a Gaussian
policy family and the Mixture Density Networks~\cite{bishop1994mixture} can be used for more powerful policy representations.

With such a formulation, the PCHID can be regarded as a method that \emph{explicitly}
learns the inverse dynamics with HID, and progressively learns the metric $\mathcal{D}(s,g)$
with Policy Continuation (PC). In this work, we justify that the approach can be extended to a more
efficient synchronous setting that \emph{implicitly} learns the inverse dynamics $\phi_s^{-1}(\cdot)$
and the derivatives of distance metric $\mathcal{D}(\cdot,\cdot)$ with regard to state $s$ at the same time. 
The key insight of our proposed method is  \emph{minimizing the First Hitting Time~\cite{alili2005representations} of a drifted random walk} (Eq.\ref{equation_4}).

Concretely, the simplest case of Eq.\ref{equation_4} is navigating in the Euclidean space, 
where the distance metric is $\mathcal{D}(s,g) = ||g-s||_2$ and the transition dynamics is an identical
mapping, \ie~$\phi_s(a) = a \in \mathcal{A}\subset \mathcal{S} $, and by applying a Gaussian
noise on the action space, we have
\begin{equation}
%\label{equation_6}
    \pi(s,g) = ds = \epsilon\frac{g-s}{||g-s||_2} \mathrm{d}t + \sigma \mathrm{d}W_t,
    \label{equation_norm_ou}
\end{equation}
which is a Stochastic Differential Equation (SDE). As our learning objective is to
increase the possibility of reaching the goal in a finite time horizon, the problem can
be formulated as minimizing the FHT 
$\tau = \inf\{{t>0: s_t = g|s_0 > g}\}$, \ie~hitting
the goal in the state space. In practice, the goal state is always a region in the
state space~\cite{plappert2018multi}, and therefore the task is to cross the region as
soon as possible.

% The learning objective is to optimize a target policy that is fully aware of the goal and therefore
% can provide optimal action from any given state toward the goal, such that
% \begin{equation}
% \label{eq_5_optimal}
%     \theta^*(s,g) = \mathop{\arg\max}_\xi \phi_s^{-1}\left(-\xi\frac{\partial \mathcal{D}(s,g)}{\partial s}\right),
% \end{equation}


%challenge is how to learn policy which has as large $\epsilon$, the goal awareness, as possible.
%Before going further for a practical algorithm, lets first have a glance at a special case of such formulation.

\subsection{Evolutionary Stochastic Policy Distillation}

As we analyzed in the previous SDE formulation, the learning objective is to minimize FHT, providing the advantage of learning k-step transitions \textbf{simutaneously}. This advantage in principle can not be used in PCHID as its PC step requires implicit curriculum to guarantee the optimality of sub-policies. 

In this section, we propose a practical algorithm that combines evolutionary
strategy with policy distillation to minimize FHT. Specifically, ESPD maintains a target deterministic policy
$\pi_T$, parameterized as a policy network, and a behavioral stochastic policy $\pi_B$
\begin{equation}
    \pi_B = \pi_T + \tilde{\eta},  \tilde{\eta}\sim\mathcal{N}(0,\sigma^2),
    \label{equation_noise}
\end{equation}
according to Eq.\ref{equation_4}, \ie~the behavior policy comes from adding a Gaussian exploration noise upon the target policy $\pi_T$, as in previous deterministic policy learning literature~\cite{lillicrap2015continuous,fujimoto2018addressing}. For the policy update step, ESPD use the evolutionary idea by distilling the well-performed behavior policies, in terms of FHT, to the target policy, instead of applying policy gradient or the zeroth-order approximation of policy gradient~\cite{salimans2017evolution} to the target policy.
\begin{algorithm}[t]
\caption{ESPD}
\label{Algorithm1}
\begin{algorithmic}
	\STATE \textbf{Require}
	\STATE ~~1.a reward function $r(s,g) = 1$ if $g = m(s)$ else $0$
	\STATE ~~2.a Horizon list $\mathcal{K} = [1,2,...,K]$
	\STATE Initialize target policy $\pi_T(s,g)$, $\pi_B(s,g) = \pi_T(s,g) + \tilde{\eta},  \tilde{\eta}\sim\mathcal{N}(0,\sigma^2)$, replay buffer $\mathcal{B} = \{\}$
	\FOR{episode $= 1,M$}
	    \STATE Generate $s_0$, $g$ by the environment
	    \FOR{$t = 1,T$}
	        \STATE Select an action by the behavior policy $a_t = \pi_B(s_t,g)$%
			\STATE Execute the action $a_t$ and get the next state $s_{t+1}$
		\ENDFOR
		\FOR{$t = 1, T$}
			%\FOR{$k \in \mathcal{K}$}
			\FOR{$k = 1, K$}
			    \STATE Calculate additional goal according to $s_{t+k}$ by $g' = m(s_{t+k})$
			    \IF{ SELECT($s_t,g'$) = True}
			        \STATE Store $(s_t,g',a_t)$ in $\mathcal{B}$
			    \ENDIF  
		    \ENDFOR
		\ENDFOR
		\STATE Sample a minibatch $B$ from buffer $\mathcal{B}$
		\STATE Optimize target policy $\pi_T(s_t,g')$ according to Eq.\ref{eq_sl}
		\STATE Update behavior policy $\pi_B = \pi_T + \tilde{\eta},  \tilde{\eta}\sim\mathcal{N}(0,\sigma^2)$
	\ENDFOR
\end{algorithmic}
\end{algorithm}
Concretely, during training, $\pi_B$ first interacts with the environment and collects a batch of transition samples, permitting us to generate a batch of HIDs, regardless of their optimality. These HIDs contain a set of transition tuples $(s,g',a)$, where $g'$ denotes the hindsight goal. \ie, the starting point, final achieved goal, and the corresponding action are included in each of these transition tuples. From an oracle-perspective, these HIDs can be regarded as generated from a series of \emph{unknown deterministic policies} instead of a known stochastic policy $\pi_B$, each provides a individual solution for the state-goal pair task $(s,g')$. Among these unknown oracle-policies, some are better than our current target policy $\pi_T$ in terms of FHT, which means they are able to solve the certain state-goal pair task in fewer steps, or they are able to solve some sub-tasks while the $\pi_T$ is not. Although we are not able to access these well-performing oracle-policies directly, we can distill the useful knowledge from them to $\pi_T$ through their corresponding HIDs.


In practice, we use a SELECT function to distinguish those HIDs that outperform $\pi_T$ and store them in a buffer $\mathcal{B} = \{(s_i,g'_i,a_i)\}_{i=1,2,...},$. The SELECT function can be implemented in different ways, (1) reset the environment to a given previous state, which is always tractable in simulation~\cite{nair2018overcoming}, (2) use classifiers, dynamic models or heuristics~\cite{sun2019policy}. In this work we adopt (1) and leave the usage of model-based SELECT functions to the future work. 
To implement (1), the SELECT function takes in an episode generated by $\pi_B$. Suppose the episode $(s_t,a_t,s_{t+1},a_{t+1},...,s_{t+k})$ is of length $k$, the SELECT function resets environment to the starting state of this episode $s_t$ and runs $\pi_T$ for up to $k$ steps, trying to reach the final achieved state $s_{t+k}$. \ie, at every step, an action of $\pi_T(s, m(s_{t+k}))$ is performed. If $\pi_T$ is \textbf{NOT} able to reach $s_{t+k}$ within $k$ steps, the corresponding transition tuple $(s_t,m(s_{t+k}),a_t)$ will be collected in the buffer $\mathcal{B}$ and $\pi_T$ will learn from these tuples later. The procedure is illustrated in Fig.\ref{illu_fig}.

Then, we can apply Stochastic Policy Distillation (SPD) to distill the knowledge from the well-performing oracle-policies to $\pi_T$ so that $\pi_T$ may evolve to be more capable to
tackle the same sub-tasks. To be specific, we use supervised learning to minimize the difference between the action stored in the HID buffer and the action $\pi_T$ predicted. The SPD is conducted as
\begin{equation}
\label{eq_sl}
    \pi_T = \mathop{\arg\min}_{\pi_T} \frac{1}{N}\sum_{i=1}^N(\pi_T(s_i,g'_i) - a_i)^2,
\end{equation}
where $(s_i, g'_i, a_i)$ are sampled from the HID buffer $\mathcal{B}$.
From this point of view, the ESPD method
is composed of evolution strategy and policy distillation, where a stochastic behavior policy $\pi_B$ acts as the perturbation on the action space and produces diverse strategies (\emph{a population}), and we choose those well-performed strategies to distill their knowledge
into $\pi_T$ (a \emph{selection}). Fig.\ref{fig0} provides an illustration of the learning pipeline and Algorithm \ref{Algorithm1} presents the detailed learning procedure of ESPD.
\begin{figure}[t]
\begin{minipage}[htbp]{1.0\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{ICML20-RL/figures/Fetch.pdf}
		\end{minipage}%
\caption{Three robotic manipulation environments. FetchPush-v1: push a block to a goal position, FetchSlide-v1: slide a puch to a goal position and FetchPickAndPlace-v1: lift a block into the air.}
\label{fig_env}
\end{figure}
\begin{figure*}[t]
\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/Push_main.pdf}
		\end{minipage}%
		\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/Slide_main.pdf}
		\end{minipage}%
		\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/PAP_main.pdf}
		\end{minipage}%
\caption{The test success rate comparison on the FetchPush-v1, FetchSlide-v1 and FetchPickAndPlace-v1 among our proposed method (ESPD), ESPD without the SELECT function (W/O Sel.) PCHID, HER and Evolution Strategy (ES).}
\label{main_results}
\end{figure*}
% \vspace{-0.1cm}
It is worth noting that the term \textit{Evolutionary} in ESPD is used to demonstrate the
\textbf{selection} procedure. Moreover, although plenty of policy gradient methods leverage action space noise in exploration~\cite{lillicrap2015continuous,schulman2017proximal,fujimoto2018addressing}, there is a clear gap between those perturbation and the evolutionary insight in our methods:
The most important difference between action space noise in ESPD and previous policy gradient methods is that ESPD regards those \textbf{stochastic variants} as from a series of unknown \textbf{oracle deterministic policies}, then use a selection function as a filter the well-performed unknown oracle policies and finally distill those transitions to the present policy. On the other hand, previous policy gradient methods do not contain such a selection step, but instead use \textbf{all} those variants to estimate the value function and improve the policy through policy gradient accordingly.

%\subsection{A Special Case: Navigation in the Euclidean Space}



% \paragraph{From the Perspective of Bias Correction}
% Aside from the previous analysis based on the special case, here we demonstrate the
% exploration factor $\sigma$ should be selected according to the perspective of bias correction.

% Algorithm 1 learns from a series of perturbations of a deterministic policy $\pi_T$ and
% gradually evolves to be competent in more sub-tasks and becomes more powerful
% when extrapolating its knowledge to solve previously unseen state-goal pairs in more general cases. As such ability comes from the supervised learning through
% policy distillation from limited samples, the learned policy is biased with regard
% to Eq.\ref{eq_5_optimal}. The evolution part of ESPD corrects such bias through
% the TEST function: only the HIDs with less bias can pass the TEST function, or the
% present target policy $\pi_T$ will outperform those HIDs in the corresponding transitions
% and those HIDs will not be collected for policy distillation. Consequently, larger $\sigma$ will lead to better off-policy exploration with a large variance while smaller ones have low variance with large bias, and can help to increase the pass-rate of the TEST function.



==> fig/ICML20-RL/5_experiments.tex <==
% !TEX root = ICML20_ESPD.tex
\section{Experiments}

\subsection{Result on the Fetch Benchmarks}

\begin{figure*}[t]
\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/Push_factor.pdf}
		\end{minipage}%
		\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/Slide_factor.pdf}
		\end{minipage}%
		\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/PAP_factor.pdf}
		\end{minipage}%

\caption{The test success rate comparison on the FetchPush-v1, FetchSlide-v1 and FetchPickAndPlace-v1 with different scale of exploration factors.}
\label{exp_factor}
\end{figure*}
\begin{figure*}[t]
\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/Push_horizon.pdf}
		\end{minipage}%
		\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/Slide_horizon.pdf}
		\end{minipage}%
		\begin{minipage}[htbp]{0.33\linewidth}
			\centering
			\includegraphics[width=1.0\linewidth]{figures/PAP_horizon.pdf}
		\end{minipage}%
\caption{The test success rate comparison on the FetchPush-v1, FetchSlide-v1 and FetchPickAndPlace-v1 with different scales of Horizon $K$.}
\label{horizon}
\end{figure*}
% \vspace{-0.1cm}
We demonstrate the proposed method on the Fetch Benchmarks. Specifically,
we evaluate our method on the FetchPush, FetchSlide and
FetchPickAndPlace environments, as shown in Fig.\ref{fig_env}. We compare our proposed method
with the HER~\cite{NIPS2017_7090,plappert2018multi} released in OpenAI
Baselines~\cite{baselines} and the Evolution Strategy~\cite{salimans2017evolution} which is a counterpart of our method with parameter noise. We also include PCHID as a baseline, however as PCHID~\cite{sun2019policy} can be regarded as a special case of ESPD if we gradually increase the hyper-parameter Horizon in ESPD from $1$ to $K$, the performance of PCHID is upper-bounded by ESPD. Such result can also be inferred from our ablation study on the Horizon $K$ in the next section, which shows smaller $K$ limits the performance, and achieves worse learning efficiency than $K=8$, the default hyper-parameter used in ESPD. 

Fig.\ref{main_results} shows the comparison of different approaches. For each environment, we conduct 5 experiments with different random seeds and plot the averaged learning curve. In Fig.\ref{main_results}, we also show the ablated experiment result by turning off the SELECT step in ESPD, where the result is denoted as W/O Sel. Such a ablation study demonstrates the importance of the SELECT step. ESPD shows superior learning efficiency and can learn to solve the task in fewer episodes in all the three environments.

\subsection{Sensitivity to Hyper-Parameter}
\paragraph{Exploration Factor}

The exploration factor $\sigma$ controls the randomness of behavior policy and therefore determines the behavior of generated samples. While larger $\sigma$ helps the agents to benefit exploration by generating samples with large variance, smaller $\sigma$ helps to generate a biased sample with little variance. Here we need to select a proper $\sigma$ to balance the variance and bias.
Fig.\ref{exp_factor} shows our ablation study on the selection of different exploration factors. The results are generated with 5 different random seeds. 
We find in all environments, the exploration factor $\sigma = 1$ provides sufficient exploration and relatively high learning efficiency.



\paragraph{Horizon $K$}
In our proposed method, the parameter of Horizon $K$ determines the maximal length of sample trajectories the policy can learn from. 
Intuitively, smaller $K$ decreases the learning efficiency as the policy is limited by its small horizon, making it hard to plan for the tasks that need more steps to solve. 
On the other hand, larger $K$ will provide a better concept of the local as well as global geometry of the state space, and thus the agent may learn to solve more challenging tasks. 
However, using large $K$ introduces more interactions with the environment, and needs more computation time.
Moreover, as the tasks normally do not need lots of steps to finish, when the Horizon is getting too large, more noisy actions will be collected and be considered as better solutions and hence impede the learning performance.
Fig.\ref{horizon} shows our ablation studies on the selection of Horizon $K$. The results are generated with 5 different random seeds. We find that $K = 8$ provides satisfying results in all of the three environments. 

It is worth noting that HID can be seen as a special case of ESPD if we gradually increase the hyper-parameter Horizon in ESPD from 1 to K.
From this perspective, as shown in Fig.\ref{horizon} where at the beginning of learning a smaller Horizon leads to bad performance, the performance of HID is upper bounded by ESPD.









%\paragraph{Over-fitting and Staleness}








==> fig/ICML20-RL/6_conclusion.tex <==
% !TEX root = ICML20_ESPD.tex
\section{Conclusion}

This work developed a practical algorithm that can evolve to solve the GCRS problems by distilling knowledge from a series of the stochastic variants of a learned agent. The key insight behind our proposed method is based on the SDE formulation of the GCRS tasks: such tasks can be solved by learning to reduce the First Hitting Time. %With such a formulation, the previous self-imitate method PCHID can be exteded to a more general synchronous setting.
Based on the formulation, we proposed the method of Evolutionary Stochastic Policy Distillation (ESPD), which is composed of an evolutionary action space perturbation, a select procedure as a filter to collect data, and a policy distillation learning step to optimize the policy. Our experiments on the OpenAI Fetch benchmarks show that the proposed method has a much improved sample efficiency as well as stability with regard to previous baseline methods, namely the PCHID, the Evolution Strategies, and Hindsight Experience Replay.




%\paragraph{Mixture Density Networks} 
%The Mixture Density Networks (MDN) was proposed by \citet{bishop1994mixture} to combine neural networks with a mixture density model. \citet{ha2018world} use MDN to tackle the uncertainty of dynamics in predicting the future hidden state, and recent applications include learning from demonstration with MDN~\citep{rahmatizadeh2018vision,thabet2019sample}, dealing with the uncertainty~\citep{choi2019distributional}, and with multiple intensions~\citep{tamar2018imitation}. 
%Intuitively, combining MDN with our proposed method will enable the policy to learn diverse solutions of a given task, rather than learning an averaged policy, thus the investigation on the combination of ESPD and MDN will be promising.
%
%
%\paragraph{Causal Inference and interaction}
%In the environment of FetchSlide, the robotic arm hit the block and the goal is to let the block slide to hit a certain region in the plane. However, in ESPD, our agent is not able to distinguish those actions that cause the motion of the block from those actions that irrelevant to the motion, and therefore noise will be introduced in the data collection. The technique of causal inference may provide help in such situations to reduce the noise and improve the performance of ESPD.






==> fig/ICML20-RL/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

